Robust Structured Statistical Estimation via Conditional Gradient Type Methods

Structured statistical estimation problems are often solved by Conditional Gradient (CG) type methods to avoid the computationally expensive projection operation. However, the existing CG type methods are not robust to data corruption. To address this, we propose to robustify CG type methods against Huber's corruption model and heavy-tailed data. First, we show that the two Pairwise CG methods are stable, i.e., do not accumulate error. Combined with robust mean gradient estimation techniques, we can therefore guarantee robustness to a wide class of problems, but now in a projection-free algorithmic framework. Next, we consider high dimensional problems. Robust mean estimation based approaches may have an unacceptably high sample complexity. When the constraint set is a $\ell_0$ norm ball, Iterative-Hard-Thresholding-based methods have been developed recently. Yet extension is non-trivial even for general sets with $O(d)$ extreme points. For setting where the feasible set has $O(\text{poly}(d))$ extreme points, we develop a novel robustness method, based on a new condition we call the Robust Atom Selection Condition (RASC). When RASC is satisfied, our method converges linearly with a corresponding statistical error, with sample complexity that scales correctly in the sparsity of the problem, rather than the ambient dimension as would be required by any approach based on robust mean estimation.

==> 3.algo_bk.tex <==
\section{Algorithm Design}

In this section, we describe how to robustify the PCG and the DICG methods.

\subsection{Robust Linear Minimization Oracle to robustify PCG and DICG}
\label{sec:robust-lmo}
% The Robust Linear Minimization Oracle (RLMO) is our work horse to robustify PCG and DICG. 
% When given an atom $\ba_i$ and a set of gradient samples $\{\bg_i\}_i^N$, RLMO perform a one-dimensional (1-d) robust mean estimation on $\{\langle \bg_j, \ba_i \rangle\}_j^N$,
% to find out the inner product value between the gradient and $\ba_i$.
% Doing so for each atom in $\Acal$, and return the minimum inner product, constitutes the RLMO.

Unlike what is typical in previous work which robustifying the gradient \cite{RDC, prasad2018robust}, Robust Linear Minimization Oracle (RLMO) directly pick the FW-atoms and Away-atoms in a robust way. Bypassing gradient robustification is feasible because CG methods use the gradient only when computing the FW-atoms and the Away-atoms.
Then naturally, instead of gradient robustness condition, the key to establish the robustness of PCG and DICG is to select the corresponding atoms up to a robustness condition, which we name Robust Atom Selection Condition (RASC) as detailed in \Cref{sec:RASC}. 
It is worth noting that RLMO is one way to establish RASC, but not the only way.


RLMO is described in \Cref{alg:robust-linear-optimization-oracle}. Given a set of atoms $\Acal$, and a target vector $\bg$, the Linear Minimization Oracle (LMO) as in vanilla CG returns $\argmin_{\ba \in \Acal} \langle \ba, \bg \rangle$. 
% One way to think of this is projecting the vector $\bg$ to all of the atoms in $\Acal$, and then pick the largest one.
Since $\bg$ is in fact the empirical mean of a random vector $\bG$, i.e. $\bg = \frac{1}{N} \sum_i^N \bg_i $, then $\langle \ba, \bg \rangle = \left\langle \ba, \frac{1}{N}\sum_i^N \bg_i \right\rangle$is just the empirical mean of a random variable $\langle \ba, \bG \rangle$.
To obtain a robust estimator of the mean of $\langle \ba, \bG \rangle$, we can use a robust one dimensional mean estimator (such as MOM or TrM as in Section \ref{sec:robust-mean-estimation}),
instead of the empirical mean estimator. After performing the robust one dimensional mean estimator to estimate $\langle \ba, \bG \rangle$ for all $\ba \in \Acal$, we pick the smallest one. To use the RLMO to find the Away-Atoms, one can just negate the target vectors. This constitute the Robust Linear Minimization Oracle.
% \TODO{Connection with robust inner product? Connection with IHT?}


\input{3.2.Robust_RLOO}

% \subsection{Robust PCG and Robust DICG}

% Intuitively, conditional gradient methods requires the knowledge of the gradient only when computing the FW-atom and the Away-atom.
% Hence, the key to establish the robustness of PCG and DICG is to select the corresponding atoms up to a robustness condition, instead of robustifing gradient, as other works do \cite{RDC, prasad2018robust}.
% Such a robustness condition is named Robust Atom Selection Condition (RASC) as detailed in \Cref{sec:RASC}. 
% It is work noting that RLMO is one way to establish RASC, but not the only way ( \Cref{sec:algo-extension}).

Find the correct FW-Atoms and Away-Atoms is the key to the convergence of the original CG methods \cite{lacoste2015global, jaggi2013revisiting, garber2016linear}.
For PCG and DICG, we show that they converge linearly to the optimal if they are able to find FW-Atoms and Away-Atoms that are \textit{good enough} - formally defined as RASC as in  \Cref{sec:meta-thm-DICG-PCG}. 
RLMO can find  FW-Atoms and Away-Atoms that satisfies RASC (\Cref{sec:RASC}).
Replacing LMO with RLMO, we  describe Robust-PCG and Robust-DICG as in Algorithm \ref{alg:robust-PCG} and \ref{alg:robust-DICG}.

\input{3.1.Robust_PCG_DICG}

\textbf{Choice of hyper-parameters.} There are two hyper-parameters.
The choice of the hyper-parameter for the one dimensional robust mean estimation (1-d robustifier) is made clear in \Cref{proposition:RLMO-implies-RASC} and the corresponding general proposition in the appendix.
The choice of the learning rate follows the convergence theorems (\Cref{thm-robust-DICG-maintext} and \ref{thm-robust-PCG-appendix} in the appendix).
The learning rate will be geometrically decreasing with respect to iteration $t$, as in \cite{garber2016linear}.
One can choose the constant factor in the learning rate as in \cite{garber2016linear}.
The geometrically decreasing part in our learning rate roughly follows the sub-optimality $F(\param_t) - F(\param^*)$, where $F(\param)$ is the population function: $\E_{(\sample, y)} f_{\param}(\sample,y)$.
While we do not have access to $F(\param_t) - F(\param^*)$, we have access to a robust estimate of the duality gap for free: $\langle \nabla F(\param_t), \param_t - \bv_t^+ \rangle$ because this is an intermediate result of RLMO. Such a duality gap is a certificate of the sub-optimality \cite{garber2016linear, hazan2012projection}, and can be used to estimate $F(\param_t) - F(\param^*)$.



\subsection{Robust Mean Estimation to robustify PCG and DICG}
\label{sec:algo-extension}
While RLMO is natural and powerful for conditional gradient (CG) type method, and help us to establish the sample complexity advantages for two corruption models (see \Cref{coro:minimax-linear-regression}), it does come with limits.
One might immediately notice that the running time of RLMO depends linearly on $|\Acal|$.
When $|\Acal|$ is exponential in $d$ or infinite, such dependence is not acceptable.

Luckily, the crux to set up the robustness of PCG and DICG is RASC, and RLMO is just one of the various way to set up RASC.

% and robust sparse mean estimation methods 
An alternative to RLMO is that, one can use a multi-dimensional robust (sparse) mean estimation methods \cite{lai2016agnostic, hsu2016loss, du2017computationally} to estimate the gradient at iteration $t$, to obtain a robust gradient $\tilde{G}_t$, as in several previous work \cite{RDC, prasad2018robust}, and then use $\tilde{G}_t$ to estimate a FW-Atom and Away-Atom.
The robust gradient estimated by these works satisfies a certain robustness condition (such as Robust Descend Condition), and we establish that these robustness condition implies RASC, as detailed in  \Cref{sec:RASC} and Appendix  \Cref{sec:RASC-be-implied}. Since RASC is satisfied, the linear convergence property of PCG and DICG is maintained.
We left the details to Appendix \Cref{appendix-sec:alg-extension}.
% One computes a robust mean estimation of the gradient $\nabla F(\param_t)$ by a robust gradient,

% \TODO{Majority Voting}


==> 8.impact_statement.tex <==
\section*{Broader Impact}

In this work, the authors intend to robustify conditional gradient type methods to solve structured statistical estimation problem, which cannot be solved robustly and efficiently simultaneously in previous research.

This paper is about robust algorithm design and analysis, targeting the big-data applications, especially when the data collected is of low quality (i.e. noisy).
Therefore, this paper bears the negative impacts of big data applications, particularly, data privacy.
The crux is to prevent the data from reaching the wrong hands. With the technology development (such as differential privacy and computer security system) and the rise of social awareness about data privacy, the negative impact could be mitigated.
On the plus side, readers could obtain more accurate information for decision making, for example in online advertisement, and avoiding systematic error in the poll study. Industry practitioners could also develop more stable machine learning systems for their recommendation system, passenger assignment for shared-transportation, etc, in the face of adversary user behavior.

Moreover, the focus of this work is on its theoretical side, where it builds up tools to robustify algorithms, and offers insights into where the robustness comes from. Therefore, as a fundamental study, it is also beneficial for interpretation of science for a general audience, and future education about optimization algorithm and statistics.

==> 9.archiv_robust_est_of_atoms.tex <==
\section{Appendix: Robust estimation of the FW-Atoms and Away-Atoms.}

\begin{lemma}
The robust linear minimization oracle (RobustLMO) and the robust away step oracle (RobustASO) as in Algorithm \TODO{} generates FW-Atom $\bvtil_t^+$ and Away-Atom $\bvtil_t^-$ such that
\end{lemma}
\begin{align*}
    % \underset{\bv \in \Acal}{\max} 
    |\langle \bG, \bvtil_t^+ - \bvtil_t^- \rangle -
    \langle \bG, \bv_t^+ - \bv_t^- \rangle|
    \leq 4 \theta h_t^{1/2} + 4 \psi,
\end{align*}
\begin{proof}
Simply re-organize the terms:
\begin{align*}
    &\langle \bG, \bvtil_t^+ - \bvtil_t^- \rangle -
    \langle \bG, \bv_t^+ - \bv_t^- \rangle \\
    = & \langle \bG, \bvtil_t^+ - \bv_t^+ \rangle -
    \langle \bG, \bvtil_t^- - \bv_t^- \rangle
\end{align*}
We first consider the first term, as the second term follows a similar treatment. 
If we perform a median of mean operation to pick $\bvtil$,
denote the mean gradient corresponding to $\bvtil_t^+$ as $G_1$ and the mean gradient corresponding to $\bv_t^+$ as $G_2$. 
% If we perform a trim operator to pick $\bvtil$,
% denote the un-trimmed gradient corresponding to $\bvtil_t^+$ as $G_1$ and the mean gradient corresponding to $\bv_t^+$ as $G_2$. 
By that property of Median of Mean construction, we know that
\begin{align*}
    | \langle \bG - \bG_1, \bvtil_t^+ \rangle | \leq \theta  h_t^{1/2} + \psi \\
    | \langle \bG - \bG_2, \bv_t^+ \rangle | \leq \theta  h_t^{1/2} + \psi \\
\end{align*}
And according to the way that we pick $\bvtil$, we have that
\begin{align*}
    \langle \bG_1, \bvtil_t^+ \rangle \leq \langle \bG_2, \bv_t^+ \rangle
\end{align*}
Then
\begin{align*}
    & 2 \langle \bG, \bvtil_t^+ - \bv_t^+ \rangle \\
    = &  \langle \bG - \bG_1, \bvtil_t^+ - \bv_t^+ \rangle +
    \langle \bG - \bG_2, \bvtil_t^+ - \bv_t^+ \rangle +
    \langle \bG_1, \bvtil_t^+ - \bv_t^+ \rangle +
    \langle \bG_2, \bvtil_t^+ - \bv_t^+ \rangle \\
    \leq & \langle \bG - \bG_1, \bvtil_t^+ - \bv_t^+ \rangle +
    \langle \bG - \bG_2, \bvtil_t^+ - \bv_t^+ \rangle +
    \langle \bG_2 - \bG_1, \bv_t^+ \rangle +
    \langle \bG_2 - \bG_1, \bvtil_t^+ \rangle \\
    % = & \langle \bG, 2 \bvtil_t^+ - 2 \bv_t^+ \rangle +
    % \langle \bG_1, - \bvtil_t^+ + \bv_t^+ - \bv_t^+ - \bvtil_t^+ \rangle +
    % \langle \bG_2,  - \bvtil_t^+ + \bv_t^+ + \bv_t^+ + \bvtil_t^+\rangle \\
    = & 2 \langle \bG,  \bvtil_t^+ -  \bv_t^+ \rangle +
    2 \langle \bG_1, - \bvtil_t^+  \rangle +
    2 \langle \bG_2,  \bv_t^+ \rangle \\
    = & 2 \langle \bG - \bG_1, \bvtil_t^+ \rangle - 2 \langle \bG - \bG_2, \bv_t^+ \rangle
\end{align*}
Hence we have
\begin{align*}
    & |\langle \bG, \bvtil_t^+ - \bv_t^+ \rangle| \\
    \leq & | \langle \bG - \bG_1, \bvtil_t^+ \rangle | + |\langle \bG - \bG_2, \bv_t^+ \rangle| \\
    \leq & 2 \theta h_t^{1/2} + 2 \psi
\end{align*}

Similarly we can show a good bound for the second term:
\begin{align*}
    \langle \bG, \bvtil_t^- - \bv_t^- \rangle
    \leq | \langle \bG - \bG_3, \bvtil_t^+ \rangle | + |\langle \bG - \bG_4, \bv_t^+ \rangle|
    \leq & 2 \theta h_t^{1/2} + 2 \psi
\end{align*}
where $\bG_3$ and $\bG_4$ are the mean gradient corresponding to $\bvtil_t^-$ and $\bv_t^-$.

Hence overall we can setup that
\begin{align*}
    % \underset{\bv \in \Acal}{\max} 
    |\langle \bG, \bvtil_t^+ - \bvtil_t^- \rangle -
    \langle \bG, \bv_t^+ - \bv_t^- \rangle|
    \leq 4 \theta h_t^{1/2} + 4 \psi.
\end{align*}

\end{proof}

==> header.tex <==
\RequirePackage{latexsym}
\RequirePackage{amsmath}
%\let\proof\relax
%\let\endproof\relax
\RequirePackage{amsthm}
\RequirePackage{amssymb}
\RequirePackage{bm}
\RequirePackage{graphicx}
\RequirePackage{subfigure}
\RequirePackage{xcolor}
\RequirePackage{algorithmic}
\RequirePackage{algorithm}

%%%% Symbols specific to this project %%%%%
\newcommand{\gradest}{\widetilde{\mathbb{\nabla}}}


\newcommand{\good}{\mathrm{Good}}
\newcommand{\bad}{\mathrm{Bad}}

\newcommand{\var}{\mathtt{var}}

\newcommand{\Thetab}{\mathbf{\Theta}}
\newcommand{\supp}{\mathtt{supp}}
\newcommand{\Xib}{\mathbf{\Xi}}
%\newcommand{\mlangle}{\mathbf{ \langle }}
%\newcommand{\mrangle}{\mathbf{ \rangle }_\mathtt{M}}

\newcommand{\minnerprod}[1]{\left\langle #1  \right\rangle_\mathtt{M}}

\newcommand{\fnorm}[1]{\left\| #1  \right\|_F}
\newcommand{\tnorm}[1]{\left\| #1  \right\|_2}
\newcommand{\onorm}[1]{\left\| #1  \right\|_1}
\newcommand{\zeronorm}[1]{\left\| #1  \right\|_0}

\newcommand{\svrg}{\mathtt{inner}}


%%%%%%%% Stock standard definitions %%%%%%%%%%%%%%%

\newcommand{\ba}{\mathbf{a}}
\newcommand{\bb}{\mathbf{b}}
\newcommand{\bc}{\mathbf{c}}
\newcommand{\bd}{\mathbf{d}}
\newcommand{\be}{\mathbf{e}}
\newcommand{\bg}{\mathbf{g}}

\newcommand{\bs}{\mathbf{s}}
\newcommand{\bt}{\mathbf{t}}
\newcommand{\bu}{\mathbf{u}}
\newcommand{\bv}{\mathbf{v}}
\newcommand{\bw}{\mathbf{w}}
\newcommand{\bx}{\bm{\beta}}
% coming
\newcommand{\sample}{\mathbf{x}}
\newcommand{\param}{\bm{\beta}}



\newcommand{\by}{\mathbf{y}}
\newcommand{\bz}{\mathbf{z}}

\newcommand{\bA}{\mathbf{A}}
\newcommand{\bB}{\mathbf{B}}
\newcommand{\bC}{\mathbf{C}}
\newcommand{\bE}{\mathbf{E}}
\newcommand{\bF}{\mathbf{F}}
\newcommand{\bG}{\mathbf{G}}
\newcommand{\bU}{\mathbf{U}}
\newcommand{\bW}{\mathbf{W}}
\newcommand{\bX}{\mathbf{X}}
\newcommand{\bY}{\mathbf{Y}}
\newcommand{\bZ}{\mathbf{Z}} 


\newcommand{\atil}{\tilde{a}}
\newcommand{\btil}{\tilde{b}}
\newcommand{\ctil}{\tilde{c}}
\newcommand{\dtil}{\tilde{d}}
\newcommand{\etil}{\tilde{e}}
\newcommand{\ftil}{\tilde{f}}
\newcommand{\gtil}{\tilde{g}}
\newcommand{\htil}{\tilde{h}}
\newcommand{\itil}{\tilde{i}}
\newcommand{\jtil}{\tilde{j}}
\newcommand{\ktil}{\tilde{k}}
\newcommand{\ltil}{\tilde{l}}
\newcommand{\mtil}{\tilde{m}}
\newcommand{\ntil}{\tilde{n}}
\newcommand{\otil}{\tilde{o}}
\newcommand{\ptil}{\tilde{p}}
\newcommand{\qtil}{\tilde{q}}
\newcommand{\rtil}{\tilde{r}}
\newcommand{\stil}{\tilde{s}}
\newcommand{\ttil}{\tilde{t}}
\newcommand{\util}{\tilde{u}}
\newcommand{\vtil}{\tilde{v}}
\newcommand{\wtil}{\tilde{w}}
\newcommand{\xtil}{\tilde{x}}
\newcommand{\ytil}{\tilde{y}}
\newcommand{\ztil}{\tilde{z}}

\newcommand{\ahat}{\hat{a}}
\newcommand{\bhat}{\hat{b}}
\newcommand{\chat}{\hat{c}}
\newcommand{\dhat}{\hat{d}}
\newcommand{\ehat}{\hat{e}}
\newcommand{\fhat}{\hat{f}}
\newcommand{\ghat}{\hat{g}}
\newcommand{\hhat}{\hat{h}}
\newcommand{\ihat}{\hat{i}}
\newcommand{\jhat}{\hat{j}}
\newcommand{\khat}{\hat{k}}
\newcommand{\lhat}{\hat{l}}
\newcommand{\mhat}{\hat{m}}
\newcommand{\nhat}{\hat{n}}
\newcommand{\ohat}{\hat{o}}
\newcommand{\phat}{\hat{p}}
\newcommand{\qhat}{\hat{q}}
\newcommand{\rhat}{\hat{r}}
\newcommand{\shat}{\hat{s}}
\newcommand{\that}{\hat{t}}
\newcommand{\uhat}{\hat{u}}
\newcommand{\vhat}{\hat{v}}
\newcommand{\what}{\hat{w}}
\newcommand{\xhat}{\hat{x}}
\newcommand{\yhat}{\hat{y}}
\newcommand{\zhat}{\hat{z}}


\newcommand{\Atil}{\tilde{A}}
\newcommand{\Btil}{\tilde{B}}
\newcommand{\Ctil}{\tilde{C}}
\newcommand{\Dtil}{\tilde{D}}
\newcommand{\Etil}{\tilde{E}}
\newcommand{\Ftil}{\tilde{F}}
\newcommand{\Gtil}{\tilde{G}}
\newcommand{\Htil}{\tilde{H}}
\newcommand{\Itil}{\tilde{I}}
\newcommand{\Jtil}{\tilde{J}}
\newcommand{\Ktil}{\tilde{K}}
\newcommand{\Ltil}{\tilde{L}}
\newcommand{\Mtil}{\tilde{M}}
\newcommand{\Ntil}{\tilde{N}}
\newcommand{\Otil}{\tilde{O}}
\newcommand{\Ptil}{\tilde{P}}
\newcommand{\Qtil}{\tilde{Q}}
\newcommand{\Rtil}{\tilde{R}}
\newcommand{\Stil}{\tilde{S}}
\newcommand{\Ttil}{\tilde{T}}
\newcommand{\Util}{\tilde{U}}
\newcommand{\Vtil}{\tilde{V}}
\newcommand{\Wtil}{\tilde{W}}
\newcommand{\Xtil}{\tilde{X}}
\newcommand{\Ytil}{\tilde{Y}}
\newcommand{\Ztil}{\tilde{Z}}


\newcommand{\bGtil}{\tilde{\mathbf{G}}}

\newcommand{\abar}{\bar{a}}
\newcommand{\bbar}{\bar{b}}
\newcommand{\cbar}{\bar{c}}
\newcommand{\dbar}{\bar{d}}
\newcommand{\ebar}{\bar{e}}
\newcommand{\fbar}{\bar{f}}
\newcommand{\gbar}{\bar{g}}
\newcommand{\hbr}{\bar{h}}
\newcommand{\ibar}{\bar{i}}
\newcommand{\jbar}{\bar{j}}
\newcommand{\kbar}{\bar{k}}
\newcommand{\lbar}{\bar{l}}
\newcommand{\mbar}{\bar{m}}
\newcommand{\nbar}{\bar{n}}
\newcommand{\obar}{\bar{o}}
\newcommand{\pbar}{\bar{p}}
\newcommand{\qbar}{\bar{q}}
\newcommand{\rbar}{\bar{r}}
\newcommand{\sbar}{\bar{s}}
\newcommand{\tbar}{\bar{t}}
\newcommand{\ubar}{\bar{u}}
\newcommand{\vbar}{\bar{v}}
\newcommand{\wbar}{\bar{w}}
\newcommand{\xbar}{\bar{x}}
\newcommand{\ybar}{\bar{y}}
\newcommand{\zbar}{\bar{z}}


\newcommand{\Abar}{\bar{A}}
\newcommand{\Bbar}{\bar{B}}
\newcommand{\Cbar}{\bar{C}}
\newcommand{\Dbar}{\bar{D}}
\newcommand{\Ebar}{\bar{E}}
\newcommand{\Fbar}{\bar{F}}
\newcommand{\Gbar}{\bar{G}}
\newcommand{\Hbar}{\bar{H}}
\newcommand{\Ibar}{\bar{I}}
\newcommand{\Jbar}{\bar{J}}
\newcommand{\Kbar}{\bar{K}}
\newcommand{\Lbar}{\bar{L}}
\newcommand{\Mbar}{\bar{M}}
\newcommand{\Nbar}{\bar{N}}
\newcommand{\Obar}{\bar{O}}
\newcommand{\Pbar}{\bar{P}}
\newcommand{\Qbar}{\bar{Q}}
\newcommand{\Rbar}{\bar{R}}
\newcommand{\Sbar}{\bar{S}}
\newcommand{\Tbar}{\bar{T}}
\newcommand{\Ubar}{\bar{U}}
\newcommand{\Vbar}{\bar{V}}
\newcommand{\Wbar}{\bar{W}}
\newcommand{\Xbar}{\bar{X}}
\newcommand{\Ybar}{\bar{Y}}
\newcommand{\Zbar}{\bar{Z}}

\newcommand{\Abbar}{\bar{\Ab}}
\newcommand{\Bbbar}{\bar{\Bb}}
\newcommand{\Cbbar}{\bar{\Cb}}
\newcommand{\Dbbar}{\bar{\Db}}
\newcommand{\Ebbar}{\bar{\Eb}}
\newcommand{\Fbbar}{\bar{\Fb}}
\newcommand{\Gbbar}{\bar{\Gb}}
\newcommand{\Hbbar}{\bar{\Hb}}
\newcommand{\Ibbar}{\bar{\Ib}}
\newcommand{\Jbbar}{\bar{\Jb}}
\newcommand{\Kbbar}{\bar{\Kb}}
\newcommand{\Lbbar}{\bar{\Lb}}
\newcommand{\Mbbar}{\bar{\Mb}}
\newcommand{\Nbbar}{\bar{\Nb}}
\newcommand{\Obbar}{\bar{\Ob}}
\newcommand{\Pbbar}{\bar{\Pb}}
\newcommand{\Qbbar}{\bar{\Qb}}
\newcommand{\Rbbar}{\bar{\Rb}}
\newcommand{\Sbbar}{\bar{\Sb}}
\newcommand{\Tbbar}{\bar{\Tb}}
\newcommand{\Ubbar}{\bar{\Ub}}
\newcommand{\Vbbar}{\bar{\Vb}}
\newcommand{\Wbbar}{\bar{\Wb}}
\newcommand{\Xbbar}{\bar{\Xb}}
\newcommand{\Ybbar}{\bar{\Yb}}
\newcommand{\Zbbar}{\bar{\Zb}}

\newcommand{\Ahat}{\hat{A}}
\newcommand{\Bhat}{\hat{B}}
\newcommand{\Chat}{\hat{C}}
\newcommand{\Dhat}{\hat{D}}
\newcommand{\Ehat}{\hat{E}}
\newcommand{\Fhat}{\hat{F}}
\newcommand{\Ghat}{\hat{G}}
\newcommand{\Hhat}{\hat{H}}
\newcommand{\Ihat}{\hat{I}}
\newcommand{\Jhat}{\hat{J}}
\newcommand{\Khat}{\hat{K}}
\newcommand{\Lhat}{\hat{L}}
\newcommand{\Mhat}{\hat{M}}
\newcommand{\Nhat}{\hat{N}}
\newcommand{\Ohat}{\hat{O}}
\newcommand{\Phat}{\hat{P}}
\newcommand{\Qhat}{\hat{Q}}
\newcommand{\Rhat}{\hat{R}}
\newcommand{\Shat}{\hat{S}}
\newcommand{\That}{\hat{T}}
\newcommand{\Uhat}{\hat{U}}
\newcommand{\Vhat}{\hat{V}}
\newcommand{\What}{\hat{W}}
\newcommand{\Xhat}{\hat{X}}
\newcommand{\Yhat}{\hat{Y}}
\newcommand{\Zhat}{\hat{Z}}

\newcommand{\Abhat}{\hat{\Ab}}
\newcommand{\Bbhat}{\hat{\Bb}}
\newcommand{\Cbhat}{\hat{\Cb}}
\newcommand{\Dbhat}{\hat{\Db}}
\newcommand{\Ebhat}{\hat{\Eb}}
\newcommand{\Fbhat}{\hat{\Fb}}
\newcommand{\Gbhat}{\hat{\Gb}}
\newcommand{\Hbhat}{\hat{\Hb}}
\newcommand{\Ibhat}{\hat{\Ib}}
\newcommand{\Jbhat}{\hat{\Jb}}
\newcommand{\Kbhat}{\hat{\Kb}}
\newcommand{\Lbhat}{\hat{\Lb}}
\newcommand{\Mbhat}{\hat{\Mb}}
\newcommand{\Nbhat}{\hat{\Nb}}
\newcommand{\Obhat}{\hat{\Ob}}
\newcommand{\Pbhat}{\hat{\Pb}}
\newcommand{\Qbhat}{\hat{\Qb}}
\newcommand{\Rbhat}{\hat{\Rb}}
\newcommand{\Sbhat}{\hat{\Sb}}
\newcommand{\Tbhat}{\hat{\Tb}}
\newcommand{\Ubhat}{\hat{\Ub}}
\newcommand{\Vbhat}{\hat{\Vb}}
\newcommand{\Wbhat}{\hat{\Wb}}
\newcommand{\Xbhat}{\hat{\Xb}}
\newcommand{\Ybhat}{\hat{\Yb}}
\newcommand{\Zbhat}{\hat{\Zb}}

\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Ical}{\mathcal{I}}
\newcommand{\Jcal}{\mathcal{J}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Lcal}{\mathcal{L}}
\newcommand{\Mcal}{\mathcal{M}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Ocal}{\mathcal{O}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{{\mathcal{S}}}
\newcommand{\Tcal}{{\mathcal{T}}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}

\newcommand{\Atilde}{\widetilde{A}}
\newcommand{\Btilde}{\widetilde{B}}
\newcommand{\Ctilde}{\widetilde{C}}
\newcommand{\Dtilde}{\widetilde{D}}
\newcommand{\Etilde}{\widetilde{E}}
\newcommand{\Ftilde}{\widetilde{F}}
\newcommand{\Gtilde}{\widetilde{G}}
\newcommand{\Htilde}{\widetilde{H}}
\newcommand{\Itilde}{\widetilde{I}}
\newcommand{\Jtilde}{\widetilde{J}}
\newcommand{\Ktilde}{\widetilde{K}}
\newcommand{\Ltilde}{\widetilde{L}}
\newcommand{\Mtilde}{\widetilde{M}}
\newcommand{\Ntilde}{\widetilde{N}}
\newcommand{\Otilde}{\widetilde{O}}
\newcommand{\Ptilde}{\widetilde{P}}
\newcommand{\Qtilde}{\widetilde{Q}}
\newcommand{\Rtilde}{\widetilde{R}}
\newcommand{\Stilde}{\widetilde{S}}
\newcommand{\Ttilde}{\widetilde{T}}
\newcommand{\Utilde}{\widetilde{U}}
\newcommand{\Vtilde}{\widetilde{V}}
\newcommand{\Wtilde}{\widetilde{W}}
\newcommand{\Xtilde}{\widetilde{X}}
\newcommand{\Ytilde}{\widetilde{Y}}
\newcommand{\Ztilde}{\widetilde{Z}}

\renewcommand{\vec}[1]{\mathbf{\boldsymbol{#1}}}

\newcommand{\avec}{\vec{a}}
\newcommand{\bvec}{\vec{b}}
\newcommand{\cvec}{\vec{c}}
\newcommand{\dvec}{\vec{d}}
\newcommand{\evec}{\vec{e}}
\newcommand{\fvec}{\vec{f}}
\newcommand{\gvec}{\vec{g}}
\newcommand{\hvec}{\vec{h}}
\newcommand{\ivec}{\vec{i}}
\newcommand{\jvec}{\vec{j}}
\newcommand{\kvec}{\vec{k}}
\newcommand{\lvec}{\vec{l}}
\newcommand{\mvec}{\vec{m}}
\newcommand{\nvec}{\vec{n}}
\newcommand{\ovec}{\vec{o}}
\newcommand{\pvec}{\vec{p}}
\newcommand{\qvec}{\vec{q}}
\newcommand{\rvec}{\vec{r}}
\newcommand{\svec}{\vec{s}}
\newcommand{\tvec}{\vec{t}}
\newcommand{\uvec}{\vec{u}}
\newcommand{\vvec}{\vec{v}}
\newcommand{\wvec}{\vec{w}}
\newcommand{\xvec}{\vec{x}}
\newcommand{\yvec}{\vec{y}}
\newcommand{\zvec}{\vec{z}}

\newcommand{\va}{\vec{a}}
\newcommand{\vecb}{\vec{b}}
\newcommand{\vc}{\vec{c}}
\newcommand{\vd}{\vec{d}}
\newcommand{\veee}{\vec{e}}
\newcommand{\vf}{\vec{f}}
\newcommand{\vg}{\vec{g}}
\newcommand{\vh}{\vec{h}}
\newcommand{\vi}{\vec{i}}
\newcommand{\vo}{\vec{o}}
\newcommand{\vp}{\vec{p}}
\newcommand{\vq}{\vec{q}}
\newcommand{\vr}{\vec{r}}
\newcommand{\vs}{\vec{s}}
\newcommand{\vt}{\vec{t}}
\newcommand{\vu}{\vec{u}}
\newcommand{\vv}{\vec{v}}
\newcommand{\vx}{\vec{x}}
\newcommand{\vw}{\vec{w}}
\newcommand{\vy}{\vec{y}}
\newcommand{\vz}{\vec{z}}

\newcommand{\Avec}{\vec{A}}
\newcommand{\Bvec}{\vec{B}}
\newcommand{\Cvec}{\vec{C}}
\newcommand{\Dvec}{\vec{D}}
\newcommand{\Evec}{\vec{E}}
\newcommand{\Fvec}{\vec{F}}
\newcommand{\Gvec}{\vec{G}}
\newcommand{\Hvec}{\vec{H}}
\newcommand{\Ivec}{\vec{I}}
\newcommand{\Jvec}{\vec{J}}
\newcommand{\Kvec}{\vec{K}}
\newcommand{\Lvec}{\vec{L}}
\newcommand{\Mvec}{\vec{M}}
\newcommand{\Nvec}{\vec{N}}
\newcommand{\Ovec}{\vec{O}}
\newcommand{\Pvec}{\vec{P}}
\newcommand{\Qvec}{\vec{Q}}
\newcommand{\Rvec}{\vec{R}}
\newcommand{\Svec}{\vec{S}}
\newcommand{\Tvec}{\vec{T}}
\newcommand{\Uvec}{\vec{U}}
\newcommand{\Vvec}{\vec{V}}
\newcommand{\Wvec}{\vec{W}}
\newcommand{\Xvec}{\vec{X}}
\newcommand{\Yvec}{\vec{Y}}
\newcommand{\Zvec}{\vec{Z}}

\newcommand{\Amat}{\Ab}
\newcommand{\Bmat}{\Bb}
\newcommand{\Cmat}{\Cb}
\newcommand{\Dmat}{\Db}
\newcommand{\Emat}{\Eb}
\newcommand{\Fmat}{\Fb}
\newcommand{\Gmat}{\Gb}
\newcommand{\Hmat}{\Hb}
\newcommand{\Imat}{\Ib}

\newcommand{\Vmat}{\Vb}
\newcommand{\Wmat}{\Wb}
\newcommand{\Xmat}{\Xb}
\newcommand{\Ymat}{\Yb}
\newcommand{\Zmat}{\Zb}


\newcommand{\yvecbar}{\bar{\vec{y}}}
\newcommand{\wvecbar}{\bar{\vec{w}}}
\newcommand{\xvecbar}{\bar{\vec{x}}}
\newcommand{\yvectil}{\tilde{\vec{y}}}
\newcommand{\yvechat}{\hat{\vec{y}}}

\renewcommand{\qedsymbol}{$\blacksquare$}

%%%%%%%% Widely accepted Sets and Symbols %%%%%%%%%%%%%%%

\newcommand{\AAA}{\mathbb{A}}
\newcommand{\CC}{\mathbb{C}} % Complex numbers
\newcommand{\E}{\mathbb{E}} % Expectation
\newcommand{\FF}{\mathbb{F}} % Fexpectation
\newcommand{\HH}{\mathbb{H}} % Arbitrary field
\newcommand{\II}{\mathbb{I}} % Delta Indicator
\newcommand{\KK}{\mathbb{K}} % Arbitrary field
\newcommand{\MM}{\mathbb{M}} % Median
\newcommand{\NN}{\mathbb{N}} % Natural numbers
\newcommand{\PP}{\mathbb{P}} % Probability
\newcommand{\QQ}{\mathbb{Q}} % Rationals
\newcommand{\RR}{\mathbb{R}} % Real numbers
\newcommand{\RRbar}{\overline{\RR}} % Real numbers
\newcommand{\SSS}{\mathbb{S}}
\newcommand{\TT}{\mathbb{T}}
\newcommand{\VV}{\mathbb{V}} % Variance
\newcommand{\XX}{\mathbb{X}}
\newcommand{\YY}{\mathbb{Y}}
\newcommand{\ZZ}{\mathbb{Z}} % Integers

%%%%%%%% Mathematical Operations %%%%%%%%%%%%%%%

\newcommand*{\mini}{\mathop{\mathrm{minimize}}}
\newcommand*{\maxi}{\mathop{\mathrm{maximize}}}
\newcommand*{\argmin}{\mathop{\mathrm{argmin}}}
\newcommand*{\argmax}{\mathop{\mathrm{argmax}}}
\newcommand*{\arginf}{\mathop{\mathrm{arginf}}}
\newcommand*{\argsup}{\mathop{\mathrm{argsup}}}
\newcommand{\sgn}{\mathop{\mathrm{sign}}}
\newcommand{\tr}{\mathop{\mathrm{tr}}}
\newcommand{\diag}{\mathop{\mathrm{diag}}}
\newcommand{\rank}{\mathop{\mathrm{rank}}}
\newcommand{\vect}{\mathop{\mathrm{vec}}}
\newcommand{\traj}{\mathop{\mathrm{Traj}}}
\newcommand{\cov}{\mathrm{Cov}}
\newcommand{\conv}{\mathrm{conv}}
\newcommand{\const}{\mathrm{constant}}
\newcommand{\dom}{\mathop{\mathrm{dom}}}
\newcommand{\ri}{\mathop{\mathrm{ri}}}
\newcommand{\cl}{\mathop{\mathrm{cl}}}
\newcommand{\intr}{\mathop{\mathrm{int}}}
\newcommand{\emp}{\mathop{\mathrm{emp}}}
\newcommand{\core}{\mathop{\mathrm{core}}}
\newcommand{\co}{\mathop{\mathrm{co}}}
\newcommand{\nnz}{\mathop{\mathrm{nnz}}}
\newcommand{\eproof}{$\null\hfill\blacksquare$}

%%%%%%%% Utility functions %%%%%%%%%%%%%%%

\newcommand{\eq}[1]{(\ref{#1})}
\newcommand{\mymatrix}[2]{\left[\begin{array}{#1} #2 \end{array}\right]}
\newcommand{\mychoose}[2]{\left(\begin{array}{c} #1 \\ #2 \end{array}\right)}
\newcommand{\mydet}[1]{\det\left[ #1 \right]}
\newcommand{\myspan}[1]{\mathrm{span}\cbr{#1}}
\newcommand{\smallfrac}[2]{{\textstyle \frac{#1}{#2}}}
\newcommand{\pwrt}[1]{\frac{\partial}{\partial #1}}
\newcommand{\ppwrt}[1]{\frac{\partial^2}{(\partial #1)^2}}
\newcommand{\aleq}{\preccurlyeq}
\newcommand{\ageq}{\succcurlyeq}

%%%%%%%% Short Forms %%%%%%%%%%%%%%%

\newcommand{\ea}{\emph{et al.}}
\newcommand{\eg}{\emph{e.g.}}
\newcommand{\ie}{\emph{i.e.}}
\newcommand{\iid}{\emph{i.i.d.}}
\newcommand{\cf}{\emph{cf.}\ }
\newcommand{\wrt}{\emph{w.r.t.}\ }

%%%%%%%% Brackets %%%%%%%%%%%%%%%

\newcommand{\rbr}[1]{\left(#1\right)}
\newcommand{\sbr}[1]{\left[#1\right]}
\newcommand{\cbr}[1]{\left\{#1\right\}}
\newcommand{\nbr}[1]{\left\|#1\right\|}
\newcommand{\abr}[1]{\left|#1\right|}
\newcommand{\abs}[1]{\left|#1\right|}
\newcommand{\floor}[1]{\left\lfloor #1 \right\rfloor}
\newcommand{\ceil}[1]{\left\lceil #1 \right\rceil}
\newcommand{\inner}[2]{\left\langle #1,#2 \right\rangle}
\newcommand{\norm}[1]{\|#1\|}
\newcommand{\ccc}[1]{|\!|\!|#1|\!|\!|}
\newcommand{\sembrack}[1]{[\![#1]\!]}

%%%%%%%%%%%%%%%  Mathematical Constants  %%%%%%%%%%%%%%%

\newcommand{\one}{\mathbf{1}}  % Identity
\newcommand{\zero}{\mathbf{0}} % Zero
\newcommand{\ind}{\boldsymbol{\mathsf{I}}}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\sqrttwo}{\sqrt{2}}
\newcommand{\invsqrttwo}{\frac{1}{\sqrt{2}}}
\newcommand{\rmd}{\ensuremath{\mathrm{d}}}

%%%%%%%% Greek Symbols %%%%%%%%%%%%%%%

\newcommand{\sigmab}{\bm{\sigma}}
\newcommand{\Sigmab}{\mathbf{\Sigma}}

\newcommand{\val}{\vec{\alpha}}
\newcommand{\vbeta}{\vec{\beta}}
\newcommand{\vde}{\vec{\delta}}
\newcommand{\vga}{\vec{\gamma}}
\newcommand{\vsig}{\vec{\sigma}}
\newcommand{\vth}{\vec{\theta}}
\newcommand{\veta}{\vec{\eta}}
\newcommand{\vnu}{\vec{\nu}}
\newcommand{\vpsi}{\vec{\psi}}
\newcommand{\vpi}{\vec{\pi}}
\newcommand{\vphi}{\vec{\phi}}
\newcommand{\vxi}{\vec{\xi}}
\newcommand{\vze}{\vec{\zeta}}

\newcommand{\valbar}{\bar{\val}}
\newcommand{\valhat}{\hat{\val}}
\newcommand{\valtil}{\tilde{\val}}
\newcommand{\vthtil}{\tilde{\vth}}
\newcommand{\vthhat}{\hat{\vth}}
\newcommand{\vthbar}{\bar{\vth}}
\newcommand{\vbetatil}{\tilde{\vbeta}}
\newcommand{\vbetahat}{\hat{\vbeta}}

\newcommand{\alphavec}{\val}
\newcommand{\alphavecbar}{\bar{\val}}
\newcommand{\alphavechat}{\hat{\val}}
\newcommand{\alphavectil}{\tilde{\val}}
\newcommand{\betavec}{\vec{\beta}}
\newcommand{\gammavec}{\vec{\gamma}}
\newcommand{\deltavec}{\vec{\delta}}
\newcommand{\etavec}{\vec{\eta}}
\newcommand{\phivec}{\vec{\phi}}
\newcommand{\psivec}{\vec{\psi}}
\newcommand{\thetavec}{\vec{\theta}}
\newcommand{\muvec}{\vec{\mu}}
\newcommand{\xivec}{\vec{\xi}}
\newcommand{\chivec}{\vec{\chi}}
\newcommand{\lambdavec}{\vec{\lambda}}

\newcommand{\alphab}{\boldsymbol{\alpha}}
\newcommand{\betab}{\boldsymbol{\beta}}
\newcommand{\gammab}{\boldsymbol{\gamma}}
\newcommand{\thetab}{\boldsymbol{\theta}}
\newcommand{\mub}{\boldsymbol{\mu}}
\newcommand{\xib}{\boldsymbol{\xi}}
\newcommand{\Deltab}{\boldsymbol{\Delta}}
\newcommand{\Pib}{\boldsymbol{\Pi}}
\newcommand{\etab}{\boldsymbol{\eta}}
\newcommand{\taub}{\boldsymbol{\tau}}
\newcommand{\lambdab}{\boldsymbol{\lambda}}
\newcommand{\pitil}{\tilde{\pi}}
\newcommand{\elltil}{\tilde{\ell}}
\newcommand{\rhob}{\boldsymbol{\rho}}

\newcommand{\delhat}{\hat{\delta}}
\newcommand{\phihat}{\hat{\phi}}
\newcommand{\delbar}{\bar{\delta}}
\newcommand{\alphahat}{\hat{\alpha}}
\newcommand{\alphatil}{\tilde{\alpha}}
\newcommand{\mubar}{\bar{\mu}}
\newcommand{\thetahat}{\hat{\theta}}
\newcommand{\thetabar}{\bar{\theta}}
\newcommand{\betahat}{\hat{\beta}}

\newcommand{\xibar}{\bar{\xi}}
\newcommand{\lambdavectil}{\tilde{\vec{\lambda}}}
\newcommand{\thetatil}{\tilde{\theta}}
\newcommand{\betatil}{\tilde{\beta}}

\newcommand{\Omegabar}{\bar{\Omega}}



\newcommand{\TODO}[1]{{\bf{\color{red}{TODO: #1}}}}

\newtheorem{theorem}{Theorem}
\newtheorem{claim}[theorem]{Claim}
\newtheorem{remark}{Remark}
\newtheorem{definition}{Definition}
\newtheorem{model}{Model}
\newtheorem{corollary}{Corollary}
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{observation}[theorem]{Observation}
\newtheorem{proposition}{Proposition}
\newtheorem{fact}[theorem]{Fact}
\newtheorem{assumption}{Assumption}
